SynergAI: Edge-to-Cloud Synergy for Architecture-Driven High-Performance Orchestration for AI Inference

The rapid evolution of Artificial Intelligence (AI) and Machine Learning (ML) has significantly heightened computational demands, particularly for inference-serving workloads. While traditional cloud-based deployments offer scalability, they face challenges such as network congestion, high energy consumption, and privacy concerns. In contrast, edge computing provides low-latency and sustainable alternatives but is constrained by limited computational resources. In this work, we introduce SynergAI, a novel framework designed for performance- and architecture-aware inference serving across heterogeneous edge-to-cloud infrastructures. Built upon a comprehensive performance characterization of modern inference engines, SynergAI integrates a combination of offline and online decision-making policies to deliver intelligent, lightweight, and architecture-aware scheduling. By dynamically allocating workloads across diverse hardware architectures, it effectively minimizes Quality of Service (QoS) violations. We implement SynergAI within a Kubernetes-based ecosystem and evaluate its efficiency. Our results demonstrate that architecture-driven inference serving enables optimized and architecture-aware deployments on emerging hardware platforms, achieving an average reduction of 2.4x in QoS violations compared to a State-of-the-Art (SotA) solution.

==> tables/power-modes.tex <==
\setlength\extrarowheight{2pt}
\begin{table}[b]
\footnotesize
\caption{Power Mode Configurations for Nvidia Jetson AGX and Xavier NX Boards \MK{@Aggelos If there is not much work in the plots later, I suggest that we sort the modes by increasing freq., or increasing power???}}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{p{0.22\columnwidth}|p{0.10\columnwidth}|p{0.25\columnwidth}|p{0.15\columnwidth}|p{0.18\columnwidth}}
\specialrule{1.5pt}{0pt}{0pt}
\cellcolor{gray!10}\textbf{Board} & \cellcolor{gray!10}\textbf{Mode} & \cellcolor{gray!10}\textbf{Max CPU Frequency (MHz)} & \cellcolor{gray!10}\textbf{Online CPUs} &
\cellcolor{gray!10}\textbf{Power Budget (W)} \\
\specialrule{1.5pt}{0pt}{0pt}

\multirow{6}{*}{\textbf{Nvidia Jetson AGX}}  
    & Mode 1 & 2266 & 8 & MAXN \\
    \cline{2-5}
    & Mode 2 & 1200 & 8  & 30 \\
    \cline{2-5}
    & Mode 3 & 1450 & 6 & 30 \\
    \cline{2-5}
    & Mode 4 & 1780 & 4 & 30 \\
    \cline{2-5}
    & Mode 5 & 2100 & 2 & 30 \\
    \cline{2-5}
    & Mode 6 & 2188 & 4 & 15 \\
    \cline{2-5}
\specialrule{1.5pt}{0pt}{0pt}

\multirow{8}{*}{\textbf{Nvidia Jetson Xavier NX}}  
    & Mode 1 & 1900 & 2 & 15 \\
    \cline{2-5}
    & Mode 2 & 1400 & 4 & 15 \\
    \cline{2-5}
    & Mode 3 & 1400 & 6 & 15 \\
    \cline{2-5}
    & Mode 4 & 1500 & 2 & 10 \\
    \cline{2-5}
    & Mode 5 & 1200 & 4 & 10 \\
    \cline{2-5}
    & Mode 6 & 1900 & 4 & 10 \\
    \cline{2-5}
    & Mode 7 & 1900 & 2 & 20 \\
    \cline{2-5}
    & Mode 8 & 1400 & 4 & 20 \\
    \cline{2-5}
    & Mode 9 & 1400 & 6 & 20 \\
    \cline{2-5}
\specialrule{1.5pt}{0pt}{0pt}
\end{tabular}
}
\label{tab:power-modes}
\end{table}

